TRIGGER: A Lightweight Universal Jamming Gripper for Aerial Grasping

This work introduces TRIGGER, the first lighTweight univeRsal jammInG Gripper for aErial gRasping. TRIGGER is an omnidirectional, landing-capable aerial grasping system with resilience and robustness to collisions and inherent passive compliance. In particular, this work presents the design, fabrication, and experimental validation of a novel, intelligent, modular, universal jamming gripper specifically designed for aerial applications. Leveraging recent developments in particle jamming and soft granular materials, TRIGGER produces 15N of holding force with only a relatively small activation force of 2.5N. Experiments show the relationship between fill ratio and activation force and reveal that adding an additive to the membrane's silicone mixture improves the holding force by up to 52%. The concept is validated by mounting TRIGGER onto a multicopter performing a pick-and-release task under laboratory conditions. Based on the experimental data, a model for robotic simulators is introduced to facilitate future controller developments.

==> acknowledgement.tex <==

\section*{Acknowledgements}
This project was partially supported by the European Commission Horizon2020 research and innovation programme, under the grant agreement No 101017258 (SESAME) and by the Luxembourg National Research Fund (FNR) 5G-SKY project (ref. C19/IS/113713801).


\section*{Conflict of Interest}
The authors declare no conflict of interest.

